Develop AI Agents for System Engineering in Factorio

Continuing advances in frontier model research are paving the way for widespread deployment of AI agents. Meanwhile, global interest in building large, complex systems in software, manufacturing, energy and logistics has never been greater. Although AI driven system engineering holds tremendous promise, the static benchmarks dominating agent evaluations today fail to capture the crucial skills required for implementing dynamic systems, such as managing uncertain trade-offs and ensuring proactive adaptability. This position paper advocates for training and evaluating AI agents' system engineering abilities through automation-oriented sandbox games-particularly Factorio. By directing research efforts in this direction, we can equip AI agents with the specialized reasoning and long-horizon planning necessary to design, maintain, and optimize tomorrow's most demanding engineering projects.

==> xsections/x2_system_design.tex <==
\section{The High-Leverage Potential of Systems Engineering}
Systems engineering focuses on the design, implementation, and management of large-scale systems that integrate hardware, software, and human processes. As many grand challenges—from clean energy to advanced manufacturing—hinge on orchestrating numerous interdependent subsystems, systems engineering represents a powerful \textit{leverage point} for AI \cite{buede2016}.

Our understanding of systems has evolved significantly over time. Early industrial breakthroughs (e.g., standardized components, assembly lines, electrification) introduced new layers of complexity by boosting production volumes, reducing costs, and extending distribution chains. In aerospace and defense projects, where massive interdisciplinary teams had to be coordinated, formal systems-engineering practices took shape \cite{madni2018}. Over the years, the rigid “waterfall” model yielded to iterative and agile methods that emphasize continuous integration and rapid feedback—trends that have become mainstream in digital ecosystems. As AI agents emerge, we anticipate yet another major shift in how systems are built and managed.

\subsection{Software System Engineering}
Software engineering epitomizes the progression from narrow, component-level tasks to broader, end-to-end management of complex systems. A new engineer typically begins by learning programming fundamentals and version control on small-scale projects. Over time, they tackle concurrency challenges and diverse integrations, eventually moving into principal engineering roles responsible for overseeing large-scale deployments, holistic performance optimizations, and reliability goals. Key practices include mastering design patterns \cite{gamma1994design, pressman2010}, routine refactoring \cite{humphrey1989, fowler1999refactoring}, and overall architecture \cite{shaw1996software, bass2012architecture}.

Translating these capabilities to AI involves building agents that maintain situational awareness across the entire software lifecycle—from initial planning to ongoing monitoring \cite{blanchard2010}. Moreover, it demands agents capable of reasoned decision-making around design trade-offs, providing solutions that align with stakeholder objectives regarding performance, cost, and reliability.

Even moderate advancements in these areas can have large-scale implications for infrastructure at both national and global levels. Yet evaluating AI’s effectiveness in system-level tasks remains challenging: requirements shift without warning, performance metrics may need continuous monitoring, and cost constraints often intersect with user satisfaction. 

Although “ML for Systems” research has achieved specialized optimizations (e.g., compiler strategies), a truly comprehensive AI agent that writes complex code, orchestrates microservices, schedules updates, and minimizes disruptions is still aspirational. Its eventual realization underscores the value of a systems-engineering mindset in developing the next generation of AI agents.

\subsection{Beyond Software: A Larger Systems View}
Systems engineering extends well beyond digital domains \cite{blanchard2010} and underpins countless aspects of modern life. The technical depth and negotiation of trade-offs in software engineering are matched—if not exceeded—by examples from:
\begin{itemize}
    \item \textbf{Transportation and Logistics.} Industries like shipping, trucking, and ridesharing; public services like trains and buses; and physical infrastructure projects such as roads, bridges, and tunnels.
    \item \textbf{Energy Infrastructure.} Spanning raw material acquisition and refinement, large-scale energy generation in specialized facilities, and the storage and distribution networks required to balance loads.
    \item \textbf{Modern Agriculture.} Covering land management (irrigation, fertilization, pest control), crop and livestock cycles, and packaging and distribution systems to deliver products to market.
    \item \textbf{Advanced Manufacturing.} Involving the creation of parts from raw materials, international supply chain coordination, and final assembly of complex products in areas like computing, biotechnology, and aerospace.
\end{itemize}

Despite their specific domains, these industries share core attributes that illustrate why systems engineering is both a universal discipline and a transferable skill set. Each involves numerous interacting components, trade-offs among cost, time, and complexity, and an undeniable need for continuous \textit{adaptation} over both short and long timescales. The importance of adaptation, in particular, is examined further in the next section.

As AI progresses, it is imperative to explore its broadest beneficial applications—particularly in physical, real-world systems, which have often been overlooked relative to software. Moravec’s Paradox notes that certain cognitive tasks are easier to automate than many physical ones. This paper does not assume an immediate shift in research priorities for embodied versus virtual agent development. Rather, it emphasizes that all systems involve both low-level and high-level engineering needs. In software, these levels revolve around text-based artifacts, enabling AI-driven engineering to operate across the entire software stack as it currently exists.

By contrast, real-world manufacturing and process-based systems often feature intricate physical components whose lower-level automation remains constrained by today’s general-purpose robotics. Consequently, AI agents in these areas may, for now, be limited to high-level roles such as system architecture and design. Still, this high-level expertise is vital to specifying dynamic arrangements of components under varying constraints and trade-offs. As robotics matures, we can anticipate AI agents that excel in both high-level system design and low-level mechanical tasks, delivering a fully optimized, end-to-end engineering capability for arbitrarily complex systems.

%The unifying aspects of systems engineering have led to standards like ISO/IEC/IEEE 15288 \cite{iso15288_2015} and the INCOSE Systems Engineering Handbook \cite{incose2015} which codify best practices for the design and maintenance of these complex environments. Model-based systems engineering (MBSE) \cite{estefan2008, weilkiens2012} further streamlines collaboration by consolidating requirements, architectures, and analytical models into a unified knowledge base (e.g., SysML \cite{friedenthal2014}). This holistic representation paves the way for AI agents to act as “co-engineers,” proposing design changes, running simulations, and updating documentation in near-real time. With the right kind of training, AI agents could potentially take moonshot projects like ``build a fusion reactor" and manage the end-to-end design, creation and maintenance of the resulting systems.


==> xsections/x3_adaptability.tex <==
\section{The Central Role of Adaptability}
Whether we consider software architectures or real-world supply chains, \textbf{adaptability} is frequently the deciding factor between success and failure. Most systems operate in environments subject to continual change—driven by new regulations, hardware upgrades, economic forces, or natural disasters. These systems are built with multiple objectives in mind, and the underlying assumptions around trade-offs can shift rapidly. Moreover, because systems invariably comprise numerous interconnected components, the likelihood that some aspect will require adaptation at any given time is effectively guaranteed.

\subsection{Theory of Adaptability in Systems and Agents}
The concept of adaptation arises from \textit{cybernetics} \cite{wiener1948}, where continuous feedback loops and communication channels help systems compensate for disturbances. In a broader sense, General System Theory \cite{bertalanffy1968} introduced the notion of \textit{open systems}, which exchange energy, matter, and information with their surroundings. Beer’s “viable system model” \cite{beer1959, beer1972} emphasizes that adaptive responses often emerge from hierarchical structures designed for \textbf{proactive} adjustments. Ashby’s \textit{law of requisite variety} \cite{ashby1956} further underscores that a system must possess sufficient internal complexity to accommodate the full range of external disruptions. In large-scale environments like supply-chain networks or energy grids, system dynamics modeling \cite{sterman2000} demonstrates how feedback loops and delays can produce complex, at times chaotic, behavior \cite{gleick1987}, making adaptability essential for managing this emergent complexity.

From the perspective of machine learning, domain adaptation \cite{redko2022domainadaptationtheory} has been studied across numerous frameworks. Themes of adaptability also surface in meta-learning for agents \cite{beck2024metareinforcementlearning}, continual learning \cite{wang2024continuallearning}, in-context learning \cite{dong2024incontextlearning}, and out-of-distribution generalization \cite{liu2023outofdistribution}. Central ideas in these fields include robust representation learning, sample-efficient techniques, and safe exploration. Looking ahead, there are significant opportunities to merge and reconcile theoretical insights on adaptability from both systems theory and machine learning.

Some parallels are already evident. For instance, minimizing local optima in Kauffman’s “rugged landscapes” \cite{kauffman1993} closely resembles balancing overfitting to familiar domains and generalizing to new ones in machine learning. Holland’s work on genetic algorithms \cite{holland1975, holland1992} further illustrates how the speed of system adaptation depends on striking the right interplay between exploration (mutation) and exploitation (selection).

\subsection{Adaptability in the Real World}
Ackoff’s perspective on messy, holistic problems \cite{ackoff1974} asserts that investing in adaptability almost always delivers long-term benefits for real-world systems, largely because the costs of failure are high and future scenarios are difficult to fully anticipate. Global events such as the COVID-19 pandemic, geopolitical conflicts, and shipping bottlenecks highlight the urgency of addressing domain shifts. Real-world systems must reroute logistics, handle sudden traffic spikes, or incorporate novel processes without extensive downtime—demonstrating why adaptability is a \textbf{core requirement} in many industries.

Several high-level factors illustrate why adaptability remains indispensable for real-world systems:
\begin{itemize}
    \item \textbf{Environmental Effects.} All systems exist within broader environments that are mostly beyond human control. Severe weather, resource depletion, erosion, and other hazards necessitate that real-world systems adapt to external conditions.
    \item \textbf{Economics and Policy.} Fluctuating prices and resource availability continually affect a system’s efficiency and viability, driven by both market dynamics and deliberate regulatory actions.
    \item \textbf{Technological Progress.} Ongoing advancements in technology mean that equilibrium states are short-lived at best. Systems must keep pace with emerging trends or risk becoming obsolete.
\end{itemize}

A key insight is that adaptability depends both on the complexity of the decisions involved and on the feasibility of implementing those decisions in practice. For instance, configuring auto-scaling infrastructure for software services is relatively straightforward, assuming the necessary resources are available. Some processes may demand difficult decision-making but straightforward implementation—such as adjusting interest rates in monetary policy. Conversely, adapting physical infrastructure (e.g., boosting semiconductor manufacturing capacity) often makes implementation the main bottleneck. Consequently, training AI agents in systems engineering should facilitate both enhanced decision-making (through informed reasoning and responsiveness) and robust implementation (via automated digital or physical labor).

In short, these scenarios exemplify \textit{complex adaptive systems} \cite{holland1975, millerpage2007}, where rapid detection of changes and swift reorganization are paramount \cite{gleick1987, arthur1994}. When designed for continual learning and endowed with adequate internal variety, such systems maintain robustness across a wide spectrum of disruptions—critical attributes for modern large-scale engineering.

==> xsections/x3_evaluation.tex <==
\section{Designing Evaluations for Systems Engineering}
We highlight core trade-offs associated with building systems, namely efficiency, scalability and adaptability. We argue that systems engineering training and evaluation environments must be \textit{dynamic} and \textit{open-ended} to adequately assess the dynamic equilibrium of these characteristics.

\subsection{Real-World Intuition}
In the design phase of a system engineering project, the focus is on delivering a proposal that meets various requirements and user preferences for features and costs. This requires deep domain expertise since many valid proposals can exist, yet have varying profiles in terms of up-front costs, maintenance costs, implementation time, complexity, regulatory compliance, scalability, and so on. Design capability is readily tested in the software industry with system design interviews that pose questions such as “How would you design a real-time collaborative word processing application like Google Docs?” or, more bluntly, “Design Google Docs.”, “Design Uber.”, “Design Twitter.”, etc. These questions are not meant to be answered in a single pass, but rather serve as a starting point for iteratively gathering requirements and proposing increasingly detailed solutions.

\begin{figure}[ht]
    \centering
    \includegraphics[width=\columnwidth]{zimages/_systems/requisite_variety3.pdf}
    \caption{\textit{The Law of Requisite Variety.} $T_1: A \rightarrow E$ and $T_2: A \rightarrow D\prime$ are trajectories of viable and unviable systems respectively over time. A system is viabile within the total state space $S$ when the variety of the environment at that time $V_E$ remains a subset of variety the system can handle $V_R$. Systems must adapt proactively ($A \rightarrow B$) to ensure this condition is met, but then also reduce variety to improve efficiency and maintainability ($D\rightarrow E$).}
    \label{fig:requisite_variety}
\end{figure}

After a real system is designed, the implementation phase begins and often never truly ends. Successful systems typically continue to expand in scope because increased outputs fuel greater demand. This pattern is evident in large software services, energy networks, and public transportation systems. Even if overall scale plateaus, there is an ongoing need for repair and maintenance—particularly in physical systems but also in software, which must periodically upgrade dependencies and refactor for performance.  Consequently, the longevity and effectiveness of a system fundamentally depend on its capacity to assimilate feedback and adapt to inevitable changes.

Because adaptability can be expensive to build in, it becomes one of the pivotal trade-offs when designing and implementing systems. Ackoff’s insights into “messy,” holistic problems \cite{ackoff1974} suggest that investing in adaptability generally leads to long-term gains, well beyond the initial concerns of scaling and maintenance. The practical implementation of adaptability relies on having feedback mechanisms. This is done through automated means like logging in software or more manually such as accepting verbal customer feedback. Using the feedback to make changes to the system is thus core to ensuring it meets expectations through key performance indicators. 

Some future scenarios are more serious and difficult to fully predict. Recent examples such as the COVID-19 pandemic required large-scale adaptations not seen since World War II, and the volatility of geopolitics—as highlighted by the conflict in Ukraine—continues to demand swift adjustments in global systems. Natural disasters like hurricanes and wildfires, technological breakthroughs such as the generative AI boom, major cybersecurity incidents, and new discoveries of key commodities further underscore the need for flexible system design.

\subsection{Supporting Theory}
Fortunately, the study of systems has long acknowledged the value of adaptability, leading to foundational frameworks that inform real-world solutions. One such lineage is \emph{cybernetics} \cite{wiener1948}, which reveals how continuous feedback loops and robust communication channels allow systems to counter external disturbances. Building on this, the “viable system model” \cite{beer1959, beer1972} emphasizes hierarchical structures that encourage \textit{proactive} responses, enabling organizations and infrastructures to pivot swiftly under changing requirements. Likewise, Ashby’s \emph{law of requisite variety} \cite{ashby1956} stresses that systems must possess enough internal complexity to handle the range of potential external disruptions. 

These same principles of adaptability can sometimes clash with the pursuit of automation, which aims to reduce complexity and boost efficiency. For instance, a mechanized assembly line can mass-produce a single product more rapidly than a human worker, yet the latter may be more versatile in producing a variety of items. In software, production-level code is often streamlined through rigid abstractions, whereas one-off scripts are less optimized but highly flexible. Even in the study of LLMs, the choice between prompt-engineering and finetuning weights reflect this same trade-off. System engineers thus face a persistent challenge of preserving \emph{dynamic equilibrium}, in which the benefits of automation and scale do not compromise a system’s capacity to adapt \cite{forrester1961industrial, holling1973resilience, sterman2000business}.

From a machine learning perspective, adaptability has been explored under many paradigms, including domain adaptation \cite{redko2022domainadaptationtheory}, meta-learning for agents \cite{beck2024metareinforcementlearning}, continual learning \cite{wang2024continuallearning}, in-context learning \cite{dong2024incontextlearning}, and out-of-distribution generalization \cite{liu2023outofdistribution}. Central themes across these fields involve developing robust representations, ensuring sample-efficient training, and promoting safe exploration. By weaving AI-driven automation into systems, we now have the opportunity to significantly enhance both efficiency and adaptability—two objectives that have traditionally been at odds.

\begin{figure}[ht]
    \centering
    \includegraphics[width=\columnwidth]{zimages/_systems/viable_system2.pdf}
    \caption{\textit{The Viable System Model.} Systems are organized into five levels which are concisely: 1. operational units, 2. coordination, 3. control, 4. future planning, and 5. identity. Longer descriptions areg
    These levels are only responsible for the \textit{variety} associated with that level and can escalate or delegate as needed (Left). A key aspect is how Level 5 effectively balances out the tension between Levels 3 and 4 which are more present- and future-focused respectively (Right).}
    \label{fig:requisite_variety}
\end{figure}

\subsection{Evaluations for AI Agents}
Recent advances in AI research have fueled efforts to build virtual agents capable of increasingly complex interactions with real-world interfaces. These developments can be seen in emerging chatbot features such as code execution, web navigation, and project artifact management. As these cognitive capabilities continue to mature, they provide a foundation for agents to meaningfully contribute to systems engineering projects. Realizing this vision, however, requires a fundamental rethinking of how we both train and evaluate virtual AI agents.

Evaluation methods for LLM-derived agents naturally began with classic NLP benchmarks, such as question answering in MMLU \cite{hendrycks2021mmlu}. They have since evolved to encompass multi-turn interaction \cite{zheng2023mtbench}, multimodality \cite{yue2024mmmu}, and external tool use \cite{zhou2023agentbench, he2024webvoyager}—capabilities expected of advanced AI agents. SWE-bench \cite{jimenez2024swebench} (and its multimodal extension \cite{yang2024swebenchmultimodalaisystems}) is likely the most challenging agent benchmark in use today. It requires agents to resolve issues in codebases by modifying multiple files and subsequently passing unit tests. Though it involves reasoning and multi-step planning, it remains a static evaluation that does not measure adaptability and the capacity to maintain dynamic equilibrium. This would hold true even for an extension of the benchmark in which agents designed a system like Google Docs and implemented it, yet never had to respond to changing requirements or circumstances.

By contrast, non-LLM-based agents have often been evaluated in \emph{dynamic} environments. This is the case for agents achieving superhuman performance in competitive games such as Go \cite{silver2017alphazero} and StarCraft II \cite{vinyals2019alphastar}, where the presence of an opponent forces rapid adaptations to both the agent’s own actions and those of adversaries. For a time, increasingly complex games appeared to be a promising route to building general intelligence, culminating in work on \textit{Minecraft} via Voyager \cite{wang2023voyager} and MineDojo \cite{fan2022minedojo}. These agents achieved goals in a \emph{dynamic}, \emph{open-ended} environment, with effectively unconstrained objectives demanding resource gathering, multi-step planning, and adaptability to emergent challenges. 


\subsection{The Ideal Evaluation Environment for Systems Engineering}
Interest in dynamic, open-ended environments waned somewhat after the advent of LLM-based generalist models. However, the rapid evolution of ChatGPT and its successors—featuring multimodality, tool-use capabilities, and ample test-time compute—opens new possibilities for resurrecting this research agenda in a more advanced form.

Based on the discussion thus far, \emph{sandbox games} appear to be the ideal setting for evaluating system engineering. They let researchers specify high-level objectives and observe an agent’s ability to break down tasks, weigh trade-offs, and implement solutions. Over time, the researcher can change these objectives or introduce disruptions, testing the agent’s capacity to maintain a healthy dynamic equilibrium through iterative adaptation. The more open-ended the sandbox, the wider the variety of conditions the agent must handle. Simulated environments additionally have the benefits of being fundamentally safer than real-world testing and can manage the trade-off between world physics complexity and scalability.

Drawing on \textit{Minecraft} as inspiration, one can envision an “ideal” environment that focuses on abstractions relevant to system engineering while omitting excessively detailed physics. Full 3D simulations can be computationally expensive and often distract from the higher-level reasoning crucial for scaling and process orchestration. Accordingly, a game environment centered on resource flows, balancing trade-offs, and long-horizon planning is preferable. Core properties of such an environment include:
\begin{itemize}
    \item \textbf{Automation.} The agent’s action space should permit automating processes and managing the associated trade-offs between efficiency and adaptability.
    \item \textbf{Complex Evaluation Metrics.} Long-horizon performance, resource usage, and resilience under partial failures become measurable, enabling richer assessments than single-turn tests.
    \item \textbf{Multi-Agent Support.} Collaboration with peers, hierarchical coordination, and competition with adversaries significantly increase complexity, further testing an agent’s capacity to adapt.
    \item \textbf{Modding Support.} Allowing users and artificial agents to create modifications or extensions fosters adaptation to out-of-distribution scenarios.
    \item \textbf{Scalability.} The environment mechanics should be at the right level of abstraction to facilitate systems reasoning, planning, and implementation without requiring excessive computational resources.
\end{itemize}

There are many candidate sandbox games—\textit{Cities: Skylines}, \textit{The Sims}, \textit{Stardew Valley}, \textit{Kerbal Space Program}, \textit{No Man's Sky}, \textit{Satisfactory}, among others—that support a form of systems engineering. Yet they each have limitations with respect to one or more of the above criteria. As the next section will show, \emph{Factorio} stands out for providing an ideal testbed for AI system engineering: its mechanics inherently encourage large-scale “megabase” building, resource management, automation, and iterative adaptation.


==> xsections/x4_factorio.tex <==
\section{Factorio as a Customizable Systems Engineering Testbed}

\subsection{Overview}
\textit{Factorio} is a 2D, top-down factory-building game that challenges players (or agents) to balance resource extraction, logistics, automation, and defense. Its emphasis on large-scale production resonates with real-world engineering, where efficiency gains often trade off against adaptability. Because Factorio already models supply flows and iterative design improvements, it naturally aligns with the needs of AI research aimed at complex system orchestration.

\subsection{Science per Minute as a Key Benchmark}
A well-known community metric, \textbf{science per minute} (SPM), serves as a succinct indicator of how efficiently a factory generates the science packs that fuel technological progress. Factories must coordinate mining, refining, assembling, and logistical pathways to keep SPM high. As expansions and new tech nodes unlock, maintaining or increasing SPM inevitably reveals bottlenecks in raw materials, transport routes, or defensive measures. By tracking SPM, researchers can distill an agent’s overall effectiveness in scaling and adapting the factory.

\subsection{Modding Ecosystem for Tailored Scenarios}
\textit{Factorio} supports extensive modding through Lua scripts and a well-documented API, enabling customized recipes, resource types, and assembly times. Researchers can craft entire tech trees to match specific industrial or exploratory visions, from advanced electronics to hypothetical energy sources. These changes can be as simple as tweaking production times or as radical as introducing wholly new supply chains. Such flexibility makes it possible to simulate highly specialized domains, testing how well AI agents handle novel constraints and orchestrate unique workflows.

\subsection{Market Pricing and Multi-Agent Interactions}
Beyond altering core recipes, mods can introduce pricing mechanisms or trading systems that inject economic elements into gameplay. Multiple agents—human or AI—might barter resources, form alliances, or compete for scarce deposits in a shared world. This transforms \textit{Factorio} from a single-player puzzle into a multi-agent environment, where negotiation and diplomacy become as important as throughput optimization. It also showcases how new in-game disruptions (like sudden price spikes or embargoes) require agents to adapt quickly, echoing the unpredictability of real markets.

\subsection{Proctor-Agent Framework}
One especially promising approach is to have a \textit{proctor} agent (or a human) set objectives and constraints, with a \textit{test-taking} agent striving to meet them. The proctor might demand a certain SPM level while limiting pollution, or require the factory to handle intermittent “resource sink” events from enemy “Biters.” Such scenarios reward proactive adaptation, as agents must balance long-term scaling with short-term emergency responses. Feedback loops from the proctor—much like regulatory oversight in real industries—ensure accountability and highlight suboptimal design choices.

\subsection{Training and Evaluation Strategies}
AI researchers have considerable latitude in deciding how to train agents. \textbf{Reinforcement learning} can leverage multiple episodes, starting from scratch each time or carrying over partial progress. Alternatively, a \textbf{multimodal} AI system might interact with the standard \textit{Factorio} interface via clicks and keystrokes, enabling near-human play. Notably, the game can run at reduced frame rates (e.g., 5~FPS), making it feasible to keep real-time feedback loops without excessive computational overhead. Meanwhile, minimal interface mods can simplify data retrieval or action dispatch if pixel-based perception proves too cumbersome.

\subsection{Implications for System Engineering Research}
Altogether, \textit{Factorio} can be molded into a dynamic sandbox that emphasizes both the high-level planning and the day-to-day adaptations characteristic of real engineering. By blending automation with evolving environmental challenges, it tests an agent’s skill in steering large-scale industrial operations while remaining flexible under shifting constraints. The ease of modding, support for multi-agent play, and detailed performance metrics such as SPM all converge to create an environment uniquely suited for studying how AI might design, automate, and sustain intricate systems. 
